Source Code Classification for Energy Efficiency in Parallel Ultra Low-Power Microcontrollers

The analysis of source code through machine learning techniques is an increasingly explored research topic aiming at increasing smartness in the software toolchain to exploit modern architectures in the best possible way. In the case of low-power, parallel embedded architectures, this means finding the configuration, for instance in terms of the number of cores, leading to minimum energy consumption. Depending on the kernel to be executed, the energy optimal scaling configuration is not trivial. While recent work has focused on general-purpose systems to learn and predict the best execution target in terms of the execution time of a snippet of code or kernel (e.g. offload OpenCL kernel on multicore CPU or GPU), in this work we focus on static compile-time features to assess if they can be successfully used to predict the minimum energy configuration on PULP, an ultra-low-power architecture featuring an on-chip cluster of RISC-V processors. Experiments show that using machine learning models on the source code to select the best energy scaling configuration automatically is viable and has the potential to be used in the context of automatic system configuration for energy minimisation.

==> sections/2-background-old.tex <==
\section{Background and Related Works}
\label{section:background}

\subsection{The Parallel Ultra-Low Power Platform}
The target architecture of this work is the Parallel Ultra-Low Power Platform (\pulp), a soft IP implementing a cluster of processors built around a parametric number of \riscy \cite{gautschi2017near} cores (up to 16).
\riscy is a RISC-V based processor with dedicated extensions for Digital Signal Processing (DSP) and machine learning workloads.
The cores share a multi-banked scratchpad memory called Tightly-Coupled Data Memory (TCDM), enabling single-cycle data access and allowing data-parallel programming models such as \openmp.
Outside the cluster, the architecture features a L2 memory hierarchy level, composed of a 15-cycle latency multi-banked scratchpad memory. 
A DMA enables data transfers between the two memory levels.

We consider a PULP instance including 8 cores, a 512 KiB L2 memory and a 64 KiB TCDM.
The cluster cores are connected to 4 Floating Point Units (FPUs), which are shared among the cores in the cluster using an interconnect that enables a fixed mapping of cores to available FPUs.
The FPU architecture is pipelined with a single stage.
This architecture, introduced in \cite{montagna2020transprecision} as \emph{8c4f1p}, is the most energy-efficient configuration of PULP; experimental results show that this solution outperforms its main competitors in the domain of embedded processing systems.

\subsection{Machine learning for source code performance estimation}

The topic of machine learning based source code analysis is gaining increasing interest in recent years.
In facts, the outbreak of complex heterogeneous architectures inspired many works which aim at exploiting source code features for predicting the device with shortest \runtime where to execute a computation.

In \cite{grewe2013} a decision tree is used for predicting whether a given \opencl kernel is most suite for running on CPU or GPU.
That work shows promising classification accuracy considering static source code features such as opcode counts, kind of memory accesses and amount of processed data.

Successively, \cite{cummins2017, barchi2019, brauckmann2020} improves accuracy results obtained by \cite{grewe2013} exploiting deep learning models based on LSTM (Long Short-Term Memory). 
Even if promising, deep learning models do not allow an insight on what static source code features are more significant for carrying out the classification task.
Moreover, their intrinsically higher complexity make them not easily trainable and more data hungry.

\subsection{Energy estimation from source code} 

Many works in the literature provide methodologies for inferring the energy consumption of an application looking at its source code, avoiding complex and time-consuming RTL simulations or measurement campaign.
While it is relatively common in High-Performance Computing (HPC) and embedded High-Performance Computing (eHPC) systems to have a power gauge, this is not the case of embedded systems where power consumption can be only accessed in a lab setting.

Such works can be divided into two families depending on how do they approach source code: methods which use dynamic features and methods that exploit static analysis.
In general, collecting dynamic features requires to run the program for accessing performance counters or the real trace of opcodes executed.
Dynamic features tend to be more accurate, but it is not always possible to collect them.
Instead, static analysis exploits metrics available without running the program, such as data-flow analysis or opcode family counts in a section of source code.

The first attempt of computing the energy required for executing a program using dynamic features is \cite{tiwari1994power}.
In that work the authors assign an average current cost to every opcode in the target ISA.
Once the program is run, the precise list of instructions executed is accessible the energy payed is esteemed. 
In \cite{kerrison2015energy} a similar approach is generalised for multi-threaded architectures.
Although these approaches provide robust energy estimations, they require the execution trace of the program to be known and refer to single-core architectures.
On the contrary, in this manuscript we aim to unveil if it is possible to predict the optimal parallelism degree directly from the static source code analysis.

The authors of \cite{benedict2015energy} exploits random forests for predicting the energy consumed by parallel \openmp applications, in the context of compiler auto-tuning. 
Such method may be able to select the most energy efficient configuration for a given program, by estimating the energy consumption for different problem sizes and active processing elements. 
However, the model proposed requires dynamic information to be used, such as wall-time and performance counter values as source code features to be considered for inferring the energetic cost of executing the input kernel.

The authors of \cite{grech2015static} present a static analysis method to predict energy consumption based on data-flow analysis.
It extracts and solves \textit{cost-relations} from the code and expresses the energy required to execute the kernel as a function of the amount of data to be processed.
\textit{Cost-relations}, annotated with the energy required for executing a basic block, approximate the energy required to execute the whole kernel.
Unfortunately, a generalisation of such methodology in multi-core environments is not available.

To the best of our knowledge, no static methods provide prediction models for detecting the optimal parallelism in \openmp applications using only static source code features.
Here, we take into account low-power multi-core environments and provide a detailed energy estimation which takes into account contention on shared resources and advanced core power management policies such as clock gating.
Moreover, we demonstrate that is possible to exploit machine code analyser tools such as LLVM-MCA in order to infer information about energy and parallelism efficiency from source code behaviour in processor microarchitectures.


==> sections/figures/static_features_count.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=6.8in]{figures/static_features_count.pdf}
    \caption{\textcolor{Red}{
        TODO
    }}
    \label{figure:static_features_count}
\end{figure*}


==> sections/tables/dataset_labels.tex <==


\begin{table}[]
\caption{\textcolor{Red}{Dataset labels unbalance}}
\label{table:dataset_labels}
\centering
\begin{tabular}{@{}lrr@{}}
 \toprule
  Label & 
  \# samples &
  \% samples \\
 \midrule
 1 &  23 &  5.1 \% \\
 2 &  29 &  6.5 \% \\
 3 &  41 &  9.2 \% \\
 4 &  41 &  9.2 \% \\
 5 &  42 &  9.4 \% \\
 6 &  46 & 10.3 \% \\
 7 &  69 & 15.6 \% \\
 8 & 155 & 34.8 \% \\
 \bottomrule
 \end{tabular}
\end{table}

